In and out of lockdown: Propagation of supply and demand shocks in a dynamic input-output model

Economic shocks due to Covid-19 were exceptional in their severity, suddenness and heterogeneity across industries. To study the upstream and downstream propagation of these industry-specific demand and supply shocks, we build a dynamic input-output model inspired by previous work on the economic response to natural disasters. We argue that standard production functions, at least in their most parsimonious parametrizations, are not adequate to model input substitutability in the context of Covid-19 shocks. We use a survey of industry analysts to evaluate, for each industry, which inputs were absolutely necessary for production over a short time period. We calibrate our model on the UK economy and study the economic effects of the lockdown that was imposed at the end of March and gradually released in May. Looking back at predictions that we released in May, we show that the model predicted aggregate dynamics very well, and sectoral dynamics to a large extent. We discuss the relative extent to which the model's dynamics and performance was due to the choice of the production function or the choice of an exogenous shock scenario. To further explore the behavior of the model, we use simpler scenarios with only demand or supply shocks, and find that popular metrics used to predict a priori the impact of shocks, such as output multipliers, are only mildly useful.

==> NEW VERSION Dynamic COVID Production Network/appendices/FO_shocks.tex <==
\section{First-order supply and demand shocks} 
\label{apx:shocks}

\subsection{Supply shocks}
Due to the Covid-19 pandemic, industries experience supply-side reductions due to the closure of non-essential industries, workers not being able to perform their activities at home, and difficulties adapting to social distancing measures. Many industries also face substantial reductions in demand. \cite{del2020supply} provide quantitative predictions of these first-order supply and demand shocks for the U.S. economy. To calculate supply-side predictions, \cite{del2020supply} constructed a Remote Labor Index, which measures the ability of different occupations to work from home, and scored industries according to their essentialness based on the Italian government regulations. 

We follow a similar approach. We score industries essentialness based on the UK government regulations and use occupational data to estimate the fraction of workers that could work remotely and the difficulties sectors faced in adapting to social distancing measures for on-site work. Several of our estimates are based on indexes and scores available for industries in the NAICS 4-digit classification system. An essential step in our methodology is to map these estimates into the WIOD industry classification system. We explain our mapping methodology below. 



\paragraph{NAICS to WIOD mapping} We build a crosswalk from the NAICS 4-digit industry classification to the classification system used in WIOD, which is a mix of ISIC 2-digit and 1-digit codes. We make this crosswalk using the NAICS to ISIC 2-digit crosswalk from the European Commission and then aggregating the 2-digit codes presented as 1-digit in the WIOD classification system. We then do an employment-weighted aggregation of the index or score in consideration from the 277 industries at the NAICS 4-digit classification level to the 55 industries in the WIOD classification. Some of the 4-digit NAICS industries map into more than one WIOD industry classification. When this happens, we assume employment is split uniformly among the WIOD industries the NAICS industry maps into. 


\paragraph{Remote Labor Index and Physical Proximity Index} To estimate the fraction of workers that could work remotely, we use the Remote Labor Index from \cite{del2020supply}. To understand the difficulties different sectors face in adapting to the social distancing measures, we compute an industry-specific Physical Proximity Index. Other works have also used the Physical Proximity of occupations to understand the economic consequences of the lockdown \citep{mongey2020workers,koren2020business}. We map the Physical Proximity Work Context\footnote{
%
https://www.onetonline.org/find/descriptor/result/4.C.2.a.3
%
} of occupations provided by O*NET into industries, using the same methodology that \cite{del2020supply} used to map the Remote Labor Index into industries. That is, we use BLS data that indicate the occupational composition of each industry and take the employment-weighted average of the occupation's work context employed in each industry at the NAICS 4-digit classification system. 
Under the assumption that the distribution of occupations across industries and that the percentage of essential workers within an industry is the same for the US and the UK, we can map the Remote Labor Index by \cite{del2020supply} and the Physical Proximity Index into the UK economy following the mapping methodology explained in the previous paragraph. The WIOD industry sector 'T' ("Activities of households as employers; undifferentiated goods- and services-producing activities of households for own use") does only maps into one NAICS code for which we do not have RLI or PPI. Since We consider  sector 'T' to be similar to the 'R\_S' sector ("Other service activities") we use the  RLI and PPI from 'R\_S' sector in the 'T' sector. In Figures~\ref{fig:RLI} and \ref{fig:PPI} we show the Remote Labor Index and the Physical Proximity Index of the WIOD sectors.



\begin{figure}%[H]
    \centering
\includegraphics[width = 0.5\textwidth]{fig/RLI_wiod.png}
    \caption{\textbf{Remote Labor Index of industries.} Remote labor index of the WIOD industry classification. See Table \ref{tab:FO_shocks_supply} for code-industry name.}
        \label{fig:RLI}
\end{figure}

\begin{figure}%[H]
    \centering
\includegraphics[width = 0.5\textwidth]{fig/PPI_wiod.png}
    \caption{\textbf{Physical Proximity Index of industries.} Physical Proximity Index of the WIOD industry classification. See Table \ref{tab:FO_shocks_supply} for code-industry name.}
        \label{fig:PPI}
\end{figure}

\paragraph{Essential score} 
To determine the essential score of industries in scenarios $S_1$ to $S_4$ we follow the UK government guidelines. We break down WIOD sectors, which are aggregates of 2-digit NACE codes, into finer 3- and 4-digit industries. The advantage of having smaller subsectors is that we can associate shutdown orders to the subsectors and then compute an average essential score for the aggregate WIOD sector. In the following, we provide some details on how we calculate essential scores while referring the reader to the online repository to check all our assumptions.
\begin{itemize}
    \item Essential score of G45 (Wholesale and retail trade and repair of motor vehicles and motorcycles). The only shops in this sector that were mandated to close were car showrooms (see footnote \ref{footn:ukleg} for a link to official legislation).  Lacking a disambiguation between retail and wholesale trade of motor vehicles, we assign a 0.5 essential score to subsector 4511, which comprises 72\% of the turnover of G45, and an essential score of 1 to all other subsectors. The average essential score for G45 turns out to be 64\%.
    \item Essential score of G47 (Retail trade, except of motor vehicles and motorcycles). All ``non-essential'' shops were mandated to close, except food and alcohol retailers, pharmacies and chemists, newsagents, homeware stores, petrol stations, bicycle shops and a few others. We assigned an essential score that could be either 0 or 1 to all 37 4-digit NACE subsectors that compose G47. Weighing essential scores by turnover results in an average essential score of 71\%.
    \item Essential score of I (Accommodation and food service activities). Almost all economic activities in this sector were mandated to close, except hotels for essential workers (e.g. those working in transportation) and workplace canteens where there is no practical alternative for staff at that workplace to obtain food. Assigning a 10\% essential score to the main hotels subsector (551) and a 50\% essential score to subsector 5629, including workplace canteens, results in an overall 5\% essential score for sector I.
     \item Essential score of R\_S (Recreational and other services). Almost all activities in this sector were mandated to close, except those related to repair, washing and funerals. Considering all 34 subsectors yields an essential score of 7\%.
\end{itemize}

\paragraph{Real Estate.} This sector includes imputed rents, which account for $69\%$ of the monetary value of the sector,\footnote{
%
\url{https://www.ons.gov.uk/economy/grossvalueaddedgva/datasets/nominalandrealregionalgrossvalueaddedbalancedbyindustry}, Table 1B.
%
}. Because we think applying a supply shock to imputed rent does not make sense, we compute that the supply shock derived from the RLI and Essential Score (which is around $50\%$) only affects $31\%$ of the sector, leading to a $15\%$ final supply shock to Real Estate (due to an error, our original work used a value of $4.7\%$).If we had used the correct real estate shock we would have predicted a 22.1\% reduction, exactly like in the data. In the main text, we still describe our prediction as having been a 21.5\% contraction, as explicitly stated in our original paper. Note that these differences are within the range of expected data revisions\footnote{see for instance \url{https://www.ons.gov.uk/economy/grossdomesticproductgdp/datasets/revisionstrianglesforukgdpabmi} for ONS GDP quarterly national accounts revisions, which are of the order of 1 pp.)}



In scenario $S_5$, we mapped the supply shocks estimated by \cite{del2020supply} at the NAICS level into the WIOD classification system as explained previously. The WIOD industry sector 'T' ("Activities of households as employers; undifferentiated goods- and services-producing activities of households for own use")  does only maps into one NAICS code for which we do not have a supply shock. Since this sector is likely to be essential, we assume a zero supply shock. 

The supply shocks at the NAICS level depend on the list of industries' essential score at the NAICS 4-digit level provided by \cite{del2020supply}.  It is important to note that, although the list of industries' essential score provided by \cite{del2020supply} is based on the Italian list of essential industries, these lists are based on different industry classification systems (NAICS and NACE, respectively) and do not have a one-to-one correspondence. To derive the essential score of industries at the NAICS level \cite{del2020supply} followed three steps. (i) the authors considered a 6-digit NAICS industry essential if the industry had correspondence with at least one essential NACE industry. (ii) \cite{del2020supply} aggregated the 6-digit NAICS essential lists into the 4-digit level taking into account the fraction of NAICS 6-digit subcategories that were considered essential. (iii) the authors revised each 4-digit NAICS industry's essential score to check for implausible classifications and reclassified ten industries whose original essential score seemed implausible. Step (i) likely resulted in a larger fraction of industries at the NAICS level to be classified as essential than in the NACE level.  This, in turn, results in supply shocks $S_5$ that are milder than they would have been if the essential score was mapped directly from NACE to WIOD and the supply shocks calculated at the WIOD level.



For scenario $S_6$ we used the list of essential industries compiled by \cite{fana2020covid} for Italy, Germany, and Spain. We make one list by taking the mean over the three countries of the essential score of each industry. This list is at the ISIC 2-digit level, which we aggregate to WIOD classification weighting each sector by its gross output in the UK.

Table \ref{tab:FO_shocks_supply} gives an overview of first-order supply shocks and Figure \ref{fig:supplyscenarios} show the supply scenarios over time.


\begin{figure}%[H]
    \centering
\includegraphics[width = \textwidth]{fig/supplyshock_scenarios.pdf}
    \caption{
    \textbf{Comparison of supply shock scenarios over time.} 
    Each panel shows industry specific supply shocks $\epsilon_{i,t}^S$ for a given scenario. The coloring of the lines is based on the same code as in Figure \ref{fig:aggregatevssectoral}. 
    }
        \label{fig:supplyscenarios}
\end{figure}

\subsection{Demand shocks}
For calibrating consumption demand shocks, we use the same data as \cite{del2020supply} which are based on the \cite{CBO2006} estimates. These estimates are available only at the more aggregate 2-digit NAICS level and map into WIOD ISIC categories without complications. To give a more detailed estimate of consumption demand shocks, we also link manufacturing sectors to the closure of certain non-essential shops as follows. 
\begin{itemize}
     \item Consumption demand shock to C13-C15 (Manufacture of textiles, wearing apparel, leather and other related products). Four subsectors (4751, 4771, 4772, 4782) selling goods produced by this manufacturing sector were mandated to close, while one subsector was permitted to remain open as it sells homeware goods (4753). Lacking more detailed information about the share of C13-C15 products that these subsectors sell, we simply give equal shares to all subsectors, leading to an 80\% consumption demand shock to C13-C15. 
      \item Consumption demand shock to C20 (Manufacture of chemicals and chemical products). Three subsectors (4752, 4773, 4774) selling homeware and medical goods were considered essential, while subsector 4775, selling cosmetic and toilet articles, was mandated to close. Using the same assumptions as above, we get a 25\% consumption demand shock for this sector.
      \end{itemize}
      The same procedure leads to consumption demand shocks for all other manufacturing subsectors.

Table \ref{tab:FO_shocks_demand} shows the demand shock for each sector and \ref{fig:demand_time} illustrates the demand shock scenarios over time.

\begin{figure}%[H]
    \centering
\includegraphics[width = \textwidth]{fig/demandshock_time.pdf}
    \caption{
    \textbf{Industry-specific demand shocks over time.} The upper left panel shows the change in preferences $\theta_{i,t}$. 
    The bottom left panel shows shock magnitudes to investment and export.
    The upper right panel shows demand shocks due to fear of unemployment $\xi_{t}$. 
    The bottom right panel is the aggregate demand shock $\tilde \epsilon_t$ taking the savings rate of 50\% into account. The coloring of the lines for industry-specific results follows the same code as in Figure \ref{fig:aggregatevssectoral}. 
    }
        \label{fig:demand_time}
\end{figure}


\input{appendices/tab_FOshocks}






==> NEW VERSION Dynamic COVID Production Network/appendices/ces_prodfun.tex <==
 \section{ Model production function and CES }
\label{apx:ces_prodfun}


Here we show that the production functions used in the main text are highly related to nested CES production functions. 
Specifically, we consider a CES production function with three nests of the form (we suppress time indices for convenience)
\begin{equation}
        x_{i}^\text{inp} = \Big( 
    a_i^\text{C} (z_i^\text{C})^\beta +
    a_i^\text{IMP} (z_i^\text{IMP})^\beta + 
    (a_i^\text{NC})^{1-\beta} (z_i^\text{NC})^\beta
    \Big)^{\frac{1}{\beta}},
\end{equation}
where $\beta$ is the substitution parameter.
Variables $a_i^\text{C} = \sum_{j \in \text{C}} A_{ji}$, 
$a_i^\text{IMP} = \sum_{j \in \text{IMP}} A_{ji} $ and
$a_i^\text{NC} = \sum_{j \in \text{NC}} A_{ji} $
are the input shares (technical coefficients) for critical, important and non-critical inputs, respectively. 
To be consistent with the specifications of the main text, we do not consider labor inputs here and only focus on $x_i^\text{inp}$. Alternatively, we could include labor inputs in the set of critical inputs and derive the full production function in an analogous manner. $z_i^\text{C}$, $z_i^\text{IMP}$ and $z_i^\text{NC}$ are CES aggregates of critical, important and non-critical inputs for which we have
\begin{align}
    z_i^\text{C} &= \left[ 
    \sum_{j \in \text{C}} A_{ji}^{1-\nu} S_{ji}^\nu
    \right]^{\frac{1}{\nu}}, \\
        z_i^\text{IMP} &= 
    \frac{1}{2}
    \left[ 
    \sum_{j \in \text{IMP}} A_{ji}^{1-\psi} S_{ji}^\psi
    \right]^{\frac{1}{\psi}} + \;
    \frac{1}{2} x_i^\text{cap}, \\
    z_i^\text{NC} &= \left[ 
    \sum_{j \in \text{NC}} A_{ji}^{1-\zeta} S_{ji}^\zeta
    \right]^{\frac{1}{\zeta}}.
\end{align}




If we assume that every input is critical (i.e. the set of important and non-critical inputs is empty: $a_i^\text{IMP} = a_i^\text{NC} = 0$), and by taking the limits $\beta, \nu \to -\infty$ we recover the Leontief production function
\begin{equation}
    x_i^\text{inp} =  
 \underset{j}{\min} \left\{ \frac{S_{ji}}{A_{ji}}
    \right\}.
\label{eq:leon_limit}
\end{equation}


If we assume that there is no critical or important inputs at all ($a_i^\text{C} = a_i^\text{IMP} = 0$), taking the limits $\beta  \to -\infty$ and $\zeta \to 1$ yields the linear production
\begin{equation}
    x_i^\text{inp} =
 \frac{ \sum_{j}  S_{ji}  }{ a_i^\text{NC} }.
\label{eq:linear_limit}
\end{equation}



The IHS1 and IHS3 production functions treat important inputs either as critical or non-critical, i.e. the set of critical inputs is again empty ($a_i^\text{IMP} = 0$). We can approximate these functions again by taking the limits $\beta, \nu \to -\infty$ and $\zeta \to 1$ which yields
\begin{equation}
    x_i^\text{inp} = \min \left\{ 
     \underset{j \in \text{C} }{\min} \left\{ \frac{S_{ji}}{A_{ji}} \right\}, 
    \frac{ \sum_{j \in \text{NC} }  S_{ji}  }{ a_i^\text{NC} }
    \right\}.
\label{eq:ihs13_limit}
\end{equation}
Note that the difference between the two production functions lies in the different definition of critical and non-critical inputs. The functional form in Eq.~\eqref{eq:ihs13_limit} applies to both cases equivalently. 

The IHS2 production function where the set of important inputs is non-empty can be similarly approximated.
In addition to the limits above, we also take the limit $\psi \rightarrow -\infty$ to obtain
\begin{equation}
    x_i^\text{inp} = \min \left\{ 
     \underset{j \in \text{C} }{\min} \left\{ \frac{S_{ji}}{A_{ji}} \right\}, 
     \frac{1}{2}
     \underset{j \in \text{IMP} }{\min} \left\{  \frac{S_{ji}}{A_{ji}} + x_i^\text{cap} \right\},
    \frac{ \sum_{j \in \text{NC} }  S_{ji}  }{ a_i^\text{NC} }
    \right\}.
\label{eq:ihs2_limit}
\end{equation}


Eqs.~\eqref{eq:ihs13_limit} and \eqref{eq:ihs2_limit} are not exactly identical to the IHS production functions used in the main text (Eqs.~\eqref{eq:xinp_ihs1} -- \eqref{eq:xinp_ihs3}), but very similar. 
The only difference is that in the IHS functions non-critical inputs do not play a role for production at all, whereas here they enter the equations as a linear term. However, simulations show that this difference is practically irrelevant. Simulating the model with the CES-derived functions instead of the IHS production functions yield exactly the same results, indicating that the linear term representing non-critical inputs is never a binding constraint.

==> NEW VERSION Dynamic COVID Production Network/appendices/ihs.tex <==
\section{Critical vs. non-critical inputs} 
\label{apx:ihs}


A survey was designed to address the question when production can continue during a lockdown.
For each industry, IHS Markit analysts were asked to rate every input of a given industry. The exact formulation of the question was as follows:
``For each industry in WIOD, please rate whether each of its inputs are essential. We will present you with an industry X and ask you to rate each input Y. The key question is: Can production continue in industry X if input Y is not available for two months?''
Analysts could rate each input according to the following allowed answers:
\begin{itemize}
    \item \textbf{0} -- This input is \textit{not} essential
    \item \textbf{1} -- This input is essential
    \item \textbf{0.5} -- This input is important but not essential
    \item \textbf{NA} -- I have no idea
\end{itemize}
To avoid confusion with the unrelated definition of essential industries which we used to calibrate first-order supply shocks, we refer to inputs as \textit{critical} and \textit{non-critical} instead of \textit{essential} and \textit{non-essential.}

Analysts were provided with the share of each input in the expenses of the industry. It was also made explicit that the ratings assume no inventories such that a rating captures the effect on production if the input is not available.

Every industry was rated by one analyst, except for industries Mining and Quarrying (B) and Manufacture of Basic Metals (C24) which were rated by three analysts. 
In case there are several ratings we took the average of the ratings and rounded it to 1 if the average was at least $2/3$ and 0 if the average was at most $1/3$. Average input ratings lying between these boundaries are assigned the value 0.5.

The ratings for each industry and input are depicted in Figure~\ref{fig:ihs_matrix}. A column denotes an industry and the corresponding rows its inputs. 
Blue colors indicate \textit{critical}, red \textit{important, but not critical} and white \textit{non-critical} inputs. Note that under the assumption of a Leontief production function every element would be considered to be critical, yielding a completely blue-colored matrix. The results shown here indicate that the majority of elements are non-critical inputs (2,338 ratings with score = 0), whereas only 477 industry-inputs are rates as critical. 365 inputs are rated as important, although not critical (score = 0.5) and \textit{NA} was assigned eleven times.

\begin{figure}[htbp]
\centering
\includegraphics[trim = {0cm 0cm 0cm 0cm}, clip,width=\textwidth]{fig/ihs/ihs_inputs_matrix.pdf}
    \caption{Criticality scores from IHS Markit analysts. 
    Rows are inputs (supply) and columns industries using these inputs (demand).
    The blue color indicates critical (score=1), red important (score=0.5) and white non-critical (score=0) inputs. Black denotes inputs which have been rated with NA. The diagonal elements are considered to be critical by definition. For industries with multiple input-ratings we took the average of all ratings and assigned a score=1 if the averaged score was at least $2/3$ and a score=0 if the average was smaller or equal to $1/3$. 
    }
    \label{fig:ihs_matrix}
\end{figure}

\begin{figure}[!htbp]
\centering
\includegraphics[trim = {0cm 0cm 0cm 0cm}, clip,width=1\textwidth]{fig/ihs/ihs_scatter_all.pdf}
    \caption{(Left panel) The figure shows how often an industry is rated as a critical input to other industries (x-axis) against the share of critical inputs this industry is using.
    The center and right panel are the same as the left panel, except for using half-critical and non-critical scores, respectively. In each plot the identity line is shown. Point sizes are proportional to gross output.
    }
    \label{fig:ihs_scatter}
\end{figure}


The left panel of Figure \ref{fig:ihs_scatter} shows for each industry how often it was rated as critical input to other industries (x-axis) and how many critical inputs this industry relies on in its own production (y-axis). Electricity and Gas (D35) are rated most frequently as critical inputs in the production of other industries (score=1 for almost 60\% of industries). Also frequently rated as critical are Land Transport (H49) and Telecommunications (J61). 
On the other hand, many manufacturing industries (ISIC codes starting with C) stand out as relying on a large number of critical inputs. For example, around 27\% of inputs to Manufacture of Coke and Refined Petroleum Products (C19) as well as to Manufacture of Chemicals (C20) are rated as critical.

The center panel of Figure \ref{fig:ihs_scatter} shows the equivalent plot for 0.5 ratings (important, but not critical inputs). Financial Services (K64) are most frequently rated as important inputs which do not necessarily stop the production of an industry if not available.
Conversely, the industry relying on many important, but not binding inputs is Wholesale and Retail Trade (G46) of which almost half of its inputs got rated with a score = 0.5.
This makes sense given that this industry heavily relies on all these inputs, but lacking one of these does not halt economic production. This case also illustrates that a Leontief production function could vastly overestimate input bottlenecks as Wholesale and Retail Trade would most likely still be able to realize output even if a several inputs were not available.

In the right panel of Figure \ref{fig:ihs_scatter} we show the same scatter plot but for non-critical inputs. 25 industries are rated to be non-critical inputs to other industries in 80\% of all cases, with Household Activities (T) and Manufacture of Furniture (C31-32) being rated as non-critical in at least 96\%.
Industries like Other Services (R-S), Other Professional, Scientific and Technical Activities (M74-75) and Administrative Activities (N) rely on mostly non-critical inputs ($>$90\%).




A detailed breakdown of the input- and industry-specific ratings are given in Table \ref{tab:ihs_results}.





\input{appendices/tab_ihs}

\FloatBarrier


==> NEW VERSION Dynamic COVID Production Network/appendices/inventory.tex <==
\section{Inventory data and calibration} 
\label{apx:inventory}

In the previous version of our work \citep{pichler2020production}, we used U.S. data from the BEA to calibrate the inventory target parameters $n_j$ in Eq. \eqref{eq:order_interm}. Here, we use more detailed UK data from the Annual Business Survey (ABS) . The ABS is the main structural business survey conducted by the ONS\footnote{ \url{ https://www.ons.gov.uk/businessindustryandtrade/business/businessservices/methodologies/annualbusinesssurveyabs}
}. It is sampled from all non-farm, non-financial private businesses in the UK (about two-thirds of the UK economy); data are available up to the 4-digit NACE level, but for our purposes 2-digit NACE industries are sufficient. The survey asks for information on a number of variables, including turnover and inventory stocks (at the beginning and end of each year). Data are available from 2008 to 2018. They show a general increase in turnover and inventory stocks (consistent with growth of the UK economy in the same period), with moderate year-on-year fluctuations.

\begin{figure}%[H]
    \centering
\includegraphics[width = \textwidth]{fig/inventory_levels.pdf}
    \caption{
    \textbf{Inventory/sales ratios over time.} 
    }
        \label{fig:inventory_levels}
\end{figure}

To proxy inventory levels available in February 2020, we proceed as follows, for each industry: (i) we take the simple average between beginning- and end-of year inventory stock levels; (ii) we calculate the ratio between this average and yearly turnover, and multiply this number by 365, because we consider a daily timescale: this inventory-to-turnover ratio is our proxy of $n_j$ (as can be seen in Figure~\ref{fig:inventory_levels}, the inventory/sales ratios are remarkably constant over time, suggesting that inventory stocks at the beginning of the Covid-19 pandemic could reliably be estimated from past data); (iii) we consider a weighted average between inventory-to-turnover ratios across all years between 2008 and 2018, giving higher weight to more recent years;\footnote{More specifically, we consider exponential weights, such that weights from a given year $X$ are proportional to $0.95^{(2018-X)}$. Some years are missing due to confidentiality problems, and data for some sectors have clear problems in some years. We deal with missing values by giving zero weights to years with missing values and renormalizing weights over the available years.} (iv) we aggregate 2-digit NACE industries to WIOD sectors (for example, we aggregate C10, C11 and C12 to C10\_C12); (v) we fill in the missing sectors (K64, K65, K66, O84, T) by imputing the average inventory-to-turnover ratio across all service sectors. 

The final inventory to sales ratios $n_j$ are shown in Figure~\ref{fig:uk_inv_sales_ratios}. As can be seen, inventories are much larger relative to sales in production, construction and trade, while they are generally lower in services, although there is considerable heterogeneity across sectors. 

\begin{figure}%[H]
    \centering
\includegraphics[width = \textwidth]{fig/uk_inv_sales_ratios.pdf}
    \caption{
    \textbf{Inventory/sales ratios for all WIOD industries.} 
    }
        \label{fig:uk_inv_sales_ratios}
\end{figure}



\newpage


==> NEW VERSION Dynamic COVID Production Network/appendices/notation.tex <==

\newpage
\section{Notation}
\label{apx:notation}

\begin{table}[H]
\scriptsize
\begin{center}
    \begin{tabular}{ | p{2cm} | p{12cm} |}
    \hline
    Symbol  & Name  \\ 
    \hline
    $N$ & Number of industries  \\
    $t$ & Time index \\
    $t_\text{start\_lockdown}$ & Start date of lockdown (March 23)\\
    $t_\text{end\_lockdown}$ & End date of lockdown (May 13) \\
    $x_{i,t}$ & Total output of industry $i$   \\
    $x_{i,t}^{\text{cap}}$ & Industry production capacity based on available labor   \\
    $x_{i,t}^{\text{inp}}$ & Industry production capacity based on available inputs   \\
    $d_{i,t}$ & Total demand for industry $i$   \\
    $Z_{ij,t}$ & Intermediate consumption of good $i$ by industry $j$  \\
    $O_{ij,t}$ & Intermediate orders (demand from industry $j$ to industry $i$)   \\
    $c_{i,t}$ & Household consumption of good $i$   \\
    $c_{i,t}^d$ & Demand of household consumption of good $i$   \\
    $f_{i,t}$ & Non-household final demand of good $i$  \\
    $f_{i,t}^d$ & Demand non-household final demand of good $i$  \\
    $l_{i,t}$ & Labor compensation to workers of industry $i$  \\
    $\tilde l_t$ & Total labor compensation    \\
    $\tilde{l}_{t}^p$ & Expectations for permanent labor income   \\
    $\tilde l^*_t$ & Total labor compensation plus social benefits   \\
    $\tilde c_t$ & Total household consumption  \\
    $\tilde{c}_{t}^d$ & Aggregate consumption demand   \\
    $n_{j}$ & Number of days of targeted inventory for industry $j$   \\
    $A_{i,j}$ & Payments to $i$ per unit produced of $j$ (technical coefficients) \\
    $S_{ij,t}$ & Stock of material $i$ held in $j$'s inventory   \\
    $\tau$ & Speed of inventory adjustment   \\
    $\theta_{i,t}$ & Share of goods from industry $i$ in consumption demand   \\
    $\bar \theta_{i,t}$ & Share of goods from industry $i$ in consumption demand (unnormalized)  \\
    $\rho$ & Speed of adjustment of aggregate consumption  \\
    $m$ & Share of labor income used to consume final domestic goods   \\
    $\xi_t$ & Fraction of pre-pandemic labor income that households expect to retain in the long-run  \\
    $\epsilon_t$ & Consumption exogenous shock   \\
    $\tilde{\epsilon}_{i}^D$ & Relative changes in demand for goods of industry $i$ during lockdown   \\
    $\tilde{\epsilon}_{i,t}$ & Relative changes in demand for goods of industry $i$   \\
    $\tilde \epsilon_t$ & Aggregate consumption shock   \\
    $\Delta l_{i,t}$ &  Desired change of labor supply of industry $i$\\
    $ l_{i,t}^\text{max}$ & Maximum labor supply for industry $i$\\
    $\gamma_\text{H}$, $\gamma_\text{F}$ & Speed of upward/downward labor adjustment (hiring/firing)  \\
    $\Delta s$ & Change in saving rate   \\
    $\nu$ & Consumption shock term representing beliefs in L-shaped recovery \\
    $b$ & Share of labor income compensated as social benefit \\
    $\text{RLI}_i$ & Remote Labor Index of industry $i$\\
    $\text{ESS}_i$ & Essential score of industry $i$\\
    $\text{PPI}_i$ & Physical Proximity Index of industry $i$\\
    $\iota$ & Scaling factor for $\text{PPI}_i$ \\ 
    $\mathcal{V}_i$ & Set of critical inputs for industry $i$\\
    $\mathcal{U}_i$ & Set of important inputs for industry $i$\\
    \hline
        \end{tabular}
\end{center}
\caption{Notation summary.}
\label{tab:notation_econ}
\scriptsize
\end{table}




==> NEW VERSION Dynamic COVID Production Network/appendices/sensitivity.tex <==
\section{Sensitivity analysis}
\label{apx:sensitivity}
To gain a better understanding of the model behavior, we conduct a series of sensitivity analyses by showing aggregate output time series under alternative parametrizations. In particular, we vary exogenous shock inputs, the production function specification and the parameters $\tau$, $\gamma_H$, $\gamma_F$ and $\Delta s$.


\paragraph{Supply shocks.}
Figure~\ref{fig:suppdemsens}(a) shows model dynamics of total output for the different supply shock scenarios considered. 
It becomes clear that alternative specifications of supply shocks can influence model results enormously. Supply shocks derived directly from the UK lockdown policy ($S_1-S_4$) yield a similar recovery pattern but nevertheless entail markedly different levels of overall impacts. When initializing the model with the shock estimates from \cite{del2020supply} ($S_5$) and \cite{fana2020covid} ($S_6$), we obtain very different dynamics.

\paragraph{Demand shocks.}
We find that our model is less sensitive with respect to changing final demand shocks within plausible ranges. Here, we compare the baseline model results with alternative specifications of consumption and ``other final demand'' (investment, export) shocks. Instead of modifying the \cite{CBO2006} consumption shocks as discussed in Section \ref{sec:consumptiondemandshockscenarios}, we now also use their raw estimates. We further consider shocks of 10\% to investment and exports which is milder than the 15\% shocks considered in the main text.
Figure~\ref{fig:suppdemsens}(a) indicates that differences are less pronounced between the alternative demand shocks compared to the supply shock scenarios, particularly during the early phase of the lockdown. Differences of several percentage points only emerge after an extended recovery period.


\begin{figure}[H]
\includegraphics[trim = {0cm 0cm 0cm 0cm}, clip, width = .95\textwidth]{fig/DEMSUP_shock_sens.pdf}
    \caption{
    \textbf{Sensitivity analysis with respect to supply and demand shocks.}
    Shocks are applied at day one. Except for supply shocks (a) and demand shocks (b), the model is initialized as in the baseline run of the main text.
    Legend (b): Raw and Main indicate the estimates from \cite{CBO2006} and its adapted version used in the main text, respectively. 15\% and 10\% refer to the two investment/export shock scenarios.
    }
        \label{fig:suppdemsens}
\end{figure}



\paragraph{Production function.}
In Figure~\ref{fig:prodfsens}(a) and (b) we show simulation results for alternative production function specifications, when using the baseline $S_4$ and the more severe $S_5$ supply shock scenarios, respectively. 
Regardless of the supply shock scenarios considered, Leontief production yields substantially more pessimistic predictions than the other production functions.
For the milder baseline supply shock scenarios, aggregate predictions are fairly similar across the other production functions, although we observe some differences after an extended period of simulation. 
Differences between the linear and IHS production functions are larger when considering the more severe shock scenario in Figure~\ref{fig:prodfsens}(b).



\begin{figure}[H]
\centering
\includegraphics[trim = {0cm 0cm 0cm 0cm}, clip, width = .95\textwidth]{fig/PRODF_shock_sens.pdf}
    \caption{
    \textbf{Sensitivity analysis with respect to production functions.}
    Shocks are applied at day one. 
    (a) is based on the $S_4$ and (b) on the $S_5$ supply shock scenario.
    Otherwise, the model is initialized as in the baseline run of the main text.
    }
        \label{fig:prodfsens}
\end{figure}



In Figure~\ref{fig:sensitivity_params} we explore model simulations with respect to different parametrizations of the inventory adjustment parameter $\tau$ (left column), hiring/firing parameters $\gamma_H$ and $\gamma_F$ (center left column), change in savings rate parameter $\Delta s$ (center right column) and consumption adjustment speed $\rho$ (right column) under alternative production function-supply shock combinations (panel rows).

\paragraph{Inventory adjustment time $\tau$.}
We find that the inventory adjustment time becomes a key parameter under Leontief production and much less so under the alternative IHS3 specification. The shorter the inventory adjustment time (smaller $\tau$), the more shocks are mitigated.
Contrary to inventory adjustment $\tau$, model results do not change much with respect to alternative specifications of $\gamma_H$ when going from Leontief production to the IHS3 function. Here, differences in model outcomes are rather due to shock severity. Model predictions are almost identical for all choices of $\gamma_H$ under mild $S_1$ shocks but differ somewhat for more substantial $S_4$ shocks. In the $S_4$ scenarios we observe that recovery is quickest for larger values of $\gamma_H$ (stiff labor markets), since firms would lose less productive capacity in the immediate aftermath of the shocks. However, this would come at the expense of reduced profits for firms which are able to more effectively reduce labor costs for smaller values of $\gamma_H$. 


\paragraph{Change in saving rate $\Delta s$.}
We find only very little variation with respect to the whole range of $\Delta s$, regardless of the underlying production function and supply shock scenario. As expected, we find the largest adverse economic impacts in case of $\Delta s = 1$, i.e. when consumers save all the extra money which they would have spent if there was no lockdown, and the mildest impacts if $\Delta s = 0$.


\paragraph{Consumption adjustment speed $\rho$.}
Similarly, the model is not very sensitive with respect to consumption adjustment speed $\rho$. The smaller $\rho$, the quicker households adjust consumption with respect to (permanent) income shocks. Note that parameter $\rho$ is based on daily time scales. Economic impacts tend to be less adverse when consumers aim to keep original consumption levels upright (large $\rho$) and more adverse if income shocks are more relevant for consumption (small $\rho$). Overall, the effects are small, in particular for the $S_1$ shock scenarios.

\begin{figure}[H]
\includegraphics[trim = {0cm 0cm 0cm 0cm}, clip, width = 1\textwidth]{fig/sensitivity_compare.pdf}
    \caption{ 
    \textbf{Results of sensitivity analysis for parameters $\tau$, $\gamma_H$, $\Delta s$ and $\rho$.}
    All plots show normalized gross output on the y-axis and days after the shocks are applied on the x-axis. Panel rows differ with respect to the combination of production function and supply shock scenario. Panel columns differ with respect to $\tau$ (left), $\gamma_H$ (center left), $\Delta s$ (center right) and $\rho$ (right) as indicated in the legend below each column. Except for the four parameters, production function and supply shock scenario, the model is initialized as in the baseline run of the main text.
    In all simulations we used $\gamma_F = 2 \gamma_H$.
    }
        \label{fig:sensitivity_params}
\end{figure}





==> NEW VERSION Dynamic COVID Production Network/appendices/tab_FOshocks.tex <==

\begin{table}[ht]
\scriptsize
\centering
\begin{tabular}{|ll|rrrrrrr|}
  \hline
ISIC & Sector & $x$ &  $\text S_1$ & $\text S_2$ & $\text S_3$ & $\text S_4$ & $\text S_5$ & $\text S_6$  \\ 
  \hline
A01 & Agriculture & 0.8 & 0.0 & 4.1 & 16.3 & 28.6 & 0.0 & 0.0 \\ 
  A02 & Forestry & 0.0 & 0.0 & 3.2 & 12.7 & 22.2 & 85.0 & 85.0 \\ 
  A03 & Fishing & 0.1 & 0.0 & 5.3 & 21.4 & 37.4 & 0.0 & 0.0 \\ 
  B & Mining & 1.3 & 0.0 & 5.2 & 20.9 & 36.6 & 35.3 & 18.4 \\ 
  C10.C12 & Manuf. Food-Beverages & 2.8 & 0.0 & 6.2 & 25.0 & 43.7 & 0.6 & 0.0 \\ 
  C13.C15 & Manuf. Textiles & 0.4 & 0.0 & 5.1 & 20.4 & 35.7 & 37.1 & 64.5 \\ 
  C16 & Manuf. Wood & 0.2 & 0.0 & 5.2 & 20.8 & 36.4 & 61.1 & 68.9 \\ 
  C17 & Manuf. Paper & 0.4 & 0.0 & 4.9 & 19.7 & 34.5 & 7.5 & 27.6 \\ 
  C18 & Media print & 0.3 & 0.0 & 4.2 & 16.7 & 29.2 & 6.0 & 0.0 \\ 
  C19 & Manuf. Coke-Petroleum & 0.9 & 0.0 & 4.7 & 18.8 & 32.9 & 18.3 & 2.1 \\ 
  C20 & Manuf. Chemical & 1.1 & 0.0 & 4.5 & 18.1 & 31.6 & 2.6 & 26.6 \\ 
  C21 & Manuf. Pharmaceutical & 0.7 & 0.0 & 4.2 & 16.8 & 29.4 & 1.1 & 0.0 \\ 
  C22 & Manuf. Rubber-Plastics & 0.7 & 0.0 & 5.3 & 21.1 & 36.9 & 28.3 & 51.0 \\ 
  C23 & Manuf. Minerals & 0.5 & 0.0 & 4.8 & 19.2 & 33.6 & 50.3 & 63.1 \\ 
  C24 & Manuf. Metals-basic & 0.6 & 0.0 & 5.4 & 21.6 & 37.8 & 57.7 & 72.6 \\ 
  C25 & Manuf. Metals-fabricated & 1.1 & 0.0 & 4.8 & 19.1 & 33.4 & 54.8 & 66.3 \\ 
  C26 & Manuf. Electronic & 0.8 & 0.0 & 2.8 & 11.4 & 19.9 & 38.5 & 41.6 \\ 
  C27 & Manuf. Electric & 0.4 & 0.0 & 4.6 & 18.3 & 32.1 & 33.3 & 58.9 \\ 
  C28 & Manuf. Machinery & 1.1 & 0.0 & 4.4 & 17.6 & 30.8 & 49.7 & 56.9 \\ 
  C29 & Manuf. Vehicles & 1.6 & 0.0 & 5.1 & 20.5 & 35.8 & 22.6 & 69.7 \\ 
  C30 & Manuf. Transport-other & 1.0 & 0.0 & 4.2 & 17.0 & 29.7 & 48.8 & 59.7 \\ 
  C31\_C32 & Manuf. Furniture & 0.6 & 0.0 & 4.8 & 19.2 & 33.5 & 36.6 & 60.5 \\ 
  C33 & Repair-Installation & 0.4 & 0.0 & 4.9 & 19.7 & 34.5 & 3.3 & 51.8 \\ 
  D35 & Electricity-Gas & 3.2 & 0.0 & 4.5 & 17.9 & 31.3 & 0.0 & 1.9 \\ 
  E36 & Water & 0.2 & 0.0 & 4.8 & 19.4 & 33.9 & 0.0 & 0.0 \\ 
  E37.E39 & Sewage & 0.8 & 0.0 & 4.8 & 19.3 & 33.8 & 0.0 & 0.0 \\ 
  F & Construction & 7.9 & 0.0 & 6.1 & 24.2 & 42.4 & 35.6 & 66.3 \\ 
  G45 & Vehicle trade & 1.7 & 19.7 & 22.4 & 30.8 & 39.1 & 31.6 & 19.7 \\ 
  G46 & Wholesale & 3.5 & 0.0 & 3.6 & 14.4 & 25.3 & 23.6 & 21.1 \\ 
  G47 & Retail & 4.7 & 14.6 & 17.8 & 27.3 & 36.8 & 30.5 & 25.2 \\ 
  H49 & Land transport & 2.0 & 0.0 & 5.3 & 21.2 & 37.1 & 11.1 & 0.0 \\ 
  H50 & Water transport & 0.6 & 0.0 & 5.7 & 22.8 & 39.9 & 12.4 & 0.0 \\ 
  H51 & Air transport & 0.6 & 0.0 & 7.1 & 28.5 & 49.9 & 0.1 & 8.1 \\ 
  H52 & Warehousing & 1.4 & 0.0 & 5.3 & 21.0 & 36.8 & 0.5 & 0.0 \\ 
  H53 & Postal & 0.7 & 0.0 & 5.1 & 20.5 & 35.9 & 0.0 & 0.0 \\ 
  I & Accommodation-Food & 2.9 & 61.4 & 61.7 & 62.7 & 63.6 & 60.8 & 63.2 \\ 
  J58 & Publishing & 0.6 & 0.0 & 2.0 & 7.9 & 13.8 & 14.4 & 2.5 \\ 
  J59\_J60 & Video-Sound-Broadcasting & 0.9 & 0.0 & 3.4 & 13.5 & 23.7 & 32.8 & 5.0 \\ 
  J61 & Telecommunications & 1.6 & 0.0 & 3.3 & 13.1 & 22.9 & 0.9 & 0.0 \\ 
  J62\_J63 & IT & 2.3 & 0.0 & 1.8 & 7.4 & 12.9 & 0.2 & 12.6 \\ 
  K64 & Finance & 4.3 & 0.0 & 1.9 & 7.6 & 13.3 & 0.0 & 0.0 \\ 
  K65 & Insurance & 3.2 & 0.0 & 1.9 & 7.5 & 13.2 & 0.0 & 0.0 \\ 
  K66 & Auxil. Finance-Insurance & 1.1 & 0.0 & 1.9 & 7.6 & 13.2 & 0.0 & 0.0 \\ 
  L68 & Real estate & 7.8 & 0.0 & 3.9 & 15.6 & 27.3 & 4.8 & 51.3 \\ 
  M69\_M70 & Legal & 2.8 & 0.0 & 2.2 & 8.9 & 15.5 & 2.0 & 18.9 \\ 
  M71 & Architecture-Engineering & 1.7 & 0.0 & 3.0 & 12.2 & 21.3 & 0.0 & 30.6 \\ 
  M72 & R\&D & 0.5 & 0.0 & 2.6 & 10.3 & 17.9 & 0.0 & 27.4 \\ 
  M73 & Advertising & 0.6 & 0.0 & 2.9 & 11.8 & 20.6 & 22.5 & 39.7 \\ 
  M74\_M75 & Other Science & 0.7 & 0.0 & 2.8 & 11.1 & 19.4 & 3.0 & 22.0 \\ 
  N & Private Administration & 4.4 & 0.0 & 5.1 & 20.5 & 36.0 & 34.9 & 51.3 \\ 
  O84 & Public Administration & 4.8 & 0.0 & 4.4 & 17.4 & 30.5 & 1.1 & 0.0 \\ 
  P85 & Education & 4.2 & 0.0 & 4.0 & 16.2 & 28.3 & 0.0 & 15.3 \\ 
  Q & Health & 7.0 & 0.0 & 6.3 & 25.3 & 44.2 & 0.1 & 0.0 \\ 
  R\_S & Other Service & 3.2 & 56.9 & 57.3 & 58.4 & 59.5 & 34.5 & 57.7 \\ 
  T & Household activities & 0.2 & 0.0 & 5.0 & 20.0 & 35.0 & 0.0 & 51.0 \\ 
   \hline
\end{tabular}
\caption{
{\bf Industry-specific supply shock details. }
Column $x$ denotes relative shares of gross output. Supply shocks $\epsilon_{i}^S$ for different scenarios are shown in the columns $\text S_1$ to $\text{S}_6$. 
%RLI stands for Remote Labor Index. ESS represents essential scores of industries based on the average of Italy, Spain and Germany, respectively.
%PPI denotes the Physical Proximity Index.
All values are in \%.
} 
\label{tab:FO_shocks_supply}
\end{table}



\begin{table}[ht]
\scriptsize
\centering
\begin{tabular}{|ll|rrrr|}
  \hline
ISIC & Sector & $c$ & $\epsilon^D_i$ & $f$  & $f$ shock \\ 
  \hline
A01 & Agriculture & 0.9 & 10.0 & 0.3 & 13.8 \\ 
  A02 & Forestry & 0.0 & 10.0 & 0.0 & 11.9 \\ 
  A03 & Fishing & 0.0 & 10.0 & 0.1 & 14.8 \\ 
  B & Mining & 0.1 & 10.0 & 1.5 & 15.3 \\ 
  C10.C12 & Manuf. Food-Beverages & 2.4 & 10.0 & 1.4 & 15.0 \\ 
  C13.C15 & Manuf. Textiles & 0.1 & 80.0 & 0.5 & 13.4 \\ 
  C16 & Manuf. Wood & 0.1 & 10.0 & 0.1 & 11.2 \\ 
  C17 & Manuf. Paper & 0.1 & 10.0 & 0.2 & 14.1 \\ 
  C18 & Media print & 0.1 & 66.0 & 0.1 & 9.4 \\ 
  C19 & Manuf. Coke-Petroleum & 1.4 & 10.0 & 0.7 & 14.8 \\ 
  C20 & Manuf. Chemical & 0.3 & 25.0 & 1.7 & 14.7 \\ 
  C21 & Manuf. Pharmaceutical & 0.3 & 10.0 & 1.2 & 14.9 \\ 
  C22 & Manuf. Rubber-Plastics & 0.1 & 10.0 & 0.6 & 14.0 \\ 
  C23 & Manuf. Minerals & 0.1 & 10.0 & 0.2 & 13.0 \\ 
  C24 & Manuf. Metals-basic & 0.0 & 10.0 & 1.7 & 15.0 \\ 
  C25 & Manuf. Metals-fabricated & 0.1 & 10.0 & 0.8 & 14.4 \\ 
  C26 & Manuf. Electronic & 0.2 & 100.0 & 1.5 & 14.9 \\ 
  C27 & Manuf. Electric & 0.1 & 10.0 & 0.8 & 14.9 \\ 
  C28 & Manuf. Machinery & 0.2 & 10.0 & 2.2 & 15.0 \\ 
  C29 & Manuf. Vehicles & 1.2 & 100.0 & 2.8 & 14.8 \\ 
  C30 & Manuf. Transport-other & 0.1 & 10.0 & 2.6 & 15.1 \\ 
  C31\_C32 & Manuf. Furniture & 0.2 & 40.0 & 0.8 & 14.7 \\ 
  C33 & Repair-Installation & 0.0 & 10.0 & 0.0 & 11.8 \\ 
  D35 & Electricity-Gas & 3.4 & 0.0 & 0.1 & 14.8 \\ 
  E36 & Water & 0.5 & 0.0 & 0.0 & 14.8 \\ 
  E37.E39 & Sewage & 0.5 & 0.0 & 1.1 & 7.6 \\ 
  F & Construction & 0.3 & 10.0 & 12.1 & 15.2 \\ 
  G45 & Vehicle trade & 1.9 & 10.0 & 0.6 & 15.0 \\ 
  G46 & Wholesale & 3.1 & 10.0 & 4.5 & 15.0 \\ 
  G47 & Retail & 15.5 & 10.0 & 0.6 & 14.1 \\ 
  H49 & Land transport & 2.5 & 67.0 & 0.2 & 14.9 \\ 
  H50 & Water transport & 0.6 & 67.0 & 0.7 & 15.0 \\ 
  H51 & Air transport & 1.2 & 67.0 & 0.5 & 15.0 \\ 
  H52 & Warehousing & 0.1 & 67.0 & 0.4 & 15.0 \\ 
  H53 & Postal & 0.1 & 0.0 & 0.1 & 14.8 \\ 
  I & Accommodation-Food & 7.9 & 80.0 & 0.8 & 15.0 \\ 
  J58 & Publishing & 0.5 & 0.0 & 0.6 & 14.7 \\ 
  J59\_J60 & Video-Sound-Broadcasting & 1.0 & 0.0 & 1.2 & 9.9 \\ 
  J61 & Telecommunications & 1.8 & 0.0 & 0.8 & 15.0 \\ 
  J62\_J63 & IT & 0.2 & 0.0 & 2.7 & 13.6 \\ 
  K64 & Finance & 3.0 & 0.0 & 3.1 & 14.9 \\ 
  K65 & Insurance & 6.0 & 0.0 & 1.6 & 14.9 \\ 
  K66 & Auxil. Finance-Insurance & 0.1 & 0.0 & 2.1 & 15.0 \\ 
  L68 & Real estate & 23.8 & 0.0 & 1.0 & 15.0 \\ 
  M69\_M70 & Legal & 0.1 & 0.0 & 1.4 & 14.4 \\ 
  M71 & Architecture-Engineering & 0.1 & 0.0 & 1.4 & 15.1 \\ 
  M72 & R\&D & 0.0 & 0.0 & 1.1 & 14.9 \\ 
  M73 & Advertising & 0.0 & 0.0 & 0.3 & 14.0 \\ 
  M74\_M75 & Other Science & 0.4 & 0.0 & 1.0 & 14.6 \\ 
  N & Private Administration & 1.0 & 0.0 & 2.8 & 14.1 \\ 
  O84 & Public Administration & 0.5 & 0.0 & 12.5 & 0.7 \\ 
  P85 & Education & 4.7 & 0.0 & 6.4 & 1.8 \\ 
  Q & Health & 3.7 & 0.0 & 14.8 & 0.2 \\ 
  R\_S & Other Service & 6.7 & 5.0 & 1.3 & 8.5 \\ 
  T & Household activities & 0.7 & 0.0 & 0.0 & 14.8 \\ 
   \hline
\end{tabular}
\caption{
{\bf Industry-specific demand shock details. }
Column $c$ denotes relative shares of final consumer consumption (which here aggregates column \emph{C1} and \emph{C2} in the WIOD) and $\epsilon_{i}^D$ represents final consumption shocks. 
Columns $f$ and $f$ \emph{shock} are relative shares of other final demand and the shocks applied to other final demand, respectively. 
All values are in \%.
} 
\label{tab:FO_shocks_demand}
\end{table}

==> NEW VERSION Dynamic COVID Production Network/appendices/tab_ihs.tex <==
\begin{table}[!htbp]
\tiny
\centering
\resizebox{1\textwidth}{!}{



\begin{tabular}{|cl|cccc|cccc|c|}
  \hline
  & & 
  \multicolumn{4}{c|}{ Input-based rankings  } &
  \multicolumn{4}{c|}{ Industry-based rankings} & \\
ISIC & Sector (abbreviated) & $1$ & $0.5$ & $0$ & NA & $1$ & $0.5$ & $0$ & NA & n \\ 
  \hline
A01 & Agriculture & 4 & 2 & 49 & 0 & 9 & 9 & 37 & 0 & 1 \\ 
  A02 & Foresty & 2 & 3 & 50 & 0 & 7 & 9 & 39 & 0 & 1 \\ 
  A03 & Fishing & 2 & 1 & 52 & 0 & 8 & 5 & 42 & 0 & 1 \\ 
  B & Mining & 7 & 1 & 47 & 0 & 9 & 2 & 44 & 0 & 3 \\ 
  C10-C12 & Manuf. Food-Beverages & 5 & 6 & 44 & 0 & 14 & 5 & 36 & 0 & 1 \\ 
  C13-C15 & Manuf. Textiles & 2 & 5 & 48 & 0 & 6 & 2 & 47 & 0 & 1 \\ 
  C16 & Manuf. Wood & 3 & 3 & 49 & 0 & 8 & 3 & 44 & 0 & 1 \\ 
  C17 & Manuf. Paper & 5 & 10 & 40 & 0 & 14 & 11 & 30 & 0 & 1 \\ 
  C18 & Media print & 3 & 6 & 46 & 0 & 6 & 3 & 46 & 0 & 1 \\ 
  C19 & Manuf. Coke-Petroleum & 18 & 4 & 33 & 0 & 15 & 6 & 33 & 2 & 1 \\ 
  C20 & Manuf. Chemical & 21 & 10 & 24 & 0 & 15 & 6 & 34 & 0 & 1 \\ 
  C21 & Manuf. Pharmaceutical & 2 & 2 & 51 & 0 & 9 & 17 & 25 & 7 & 1 \\ 
  C22 & Manuf. Rubber-Plastics & 11 & 7 & 37 & 0 & 14 & 5 & 36 & 0 & 1 \\ 
  C23 & Manuf. Minerals & 8 & 2 & 44 & 2 & 7 & 1 & 47 & 0 & 1 \\ 
  C24 & Manuf. Metals-basic & 8 & 2 & 45 & 0 & 12 & 7 & 36 & 0 & 3 \\ 
  C25 & Manuf. Metals-fabricated & 12 & 4 & 39 & 0 & 5 & 3 & 47 & 0 & 1 \\ 
  C26 & Manuf. Electronic & 10 & 7 & 38 & 0 & 14 & 10 & 31 & 0 & 1 \\ 
  C27 & Manuf. Electric & 7 & 6 & 42 & 0 & 13 & 9 & 33 & 0 & 1 \\ 
  C28 & Manuf. Machinery & 10 & 12 & 32 & 2 & 5 & 1 & 49 & 0 & 1 \\ 
  C29 & Manuf. Vehicles & 4 & 5 & 46 & 0 & 14 & 10 & 31 & 0 & 1 \\ 
  C30 & Manuf. Transport-other & 2 & 6 & 47 & 0 & 12 & 10 & 33 & 0 & 1 \\ 
  C31\_C32 & Manuf. Furniture & 1 & 1 & 53 & 0 & 8 & 4 & 43 & 0 & 1 \\ 
  C33 & Repair-Installation & 17 & 9 & 29 & 0 & 8 & 2 & 45 & 0 & 1 \\ 
  D35 & Electricity-Gas & 31 & 3 & 21 & 0 & 10 & 5 & 40 & 0 & 1 \\ 
  E36 & Water & 19 & 3 & 33 & 0 & 4 & 5 & 46 & 0 & 1 \\ 
  E37-E39 & Sewage & 18 & 3 & 34 & 0 & 6 & 8 & 41 & 0 & 1 \\ 
  F & Construction & 5 & 3 & 47 & 0 & 14 & 9 & 32 & 0 & 1 \\ 
  G45 & Vehicle trade & 2 & 5 & 48 & 0 & 9 & 7 & 39 & 0 & 1 \\ 
  G46 & Wholesale & 19 & 3 & 33 & 0 & 4 & 25 & 26 & 0 & 1 \\ 
  G47 & Retail & 2 & 3 & 50 & 0 & 6 & 10 & 39 & 0 & 1 \\ 
  H49 & Land transport & 28 & 3 & 24 & 0 & 11 & 2 & 42 & 0 & 1 \\ 
  H50 & Water transport & 9 & 8 & 38 & 0 & 8 & 5 & 42 & 0 & 1 \\ 
  H51 & Air transport & 5 & 7 & 43 & 0 & 10 & 6 & 39 & 0 & 1 \\ 
  H52 & Warehousing & 12 & 9 & 34 & 0 & 9 & 7 & 39 & 0 & 1 \\ 
  H53 & Postal & 6 & 7 & 41 & 2 & 3 & 5 & 47 & 0 & 1 \\ 
  I & Accommodation-Food & 5 & 3 & 47 & 0 & 7 & 6 & 42 & 0 & 1 \\ 
  J58 & Publishing & 1 & 2 & 52 & 0 & 10 & 14 & 31 & 0 & 1 \\ 
  J59\_J60 & Video-Sound-Broadcasting & 2 & 2 & 51 & 0 & 9 & 5 & 37 & 7 & 1 \\ 
  J61 & Telecommunications & 26 & 11 & 18 & 0 & 7 & 5 & 42 & 2 & 1 \\ 
  J62\_J63 & IT & 16 & 13 & 26 & 0 & 7 & 6 & 42 & 0 & 1 \\ 
  K64 & Finance & 10 & 19 & 26 & 0 & 6 & 3 & 46 & 0 & 1 \\ 
  K65 & Insurance & 6 & 12 & 36 & 2 & 6 & 3 & 46 & 0 & 1 \\ 
  K66 & Auxil. Finance-Insurance & 5 & 7 & 41 & 4 & 6 & 4 & 45 & 0 & 1 \\ 
  L68 & Real estate & 1 & 3 & 51 & 0 & 7 & 5 & 43 & 0 & 1 \\ 
  M69\_M70 & Legal & 12 & 15 & 28 & 0 & 5 & 3 & 46 & 2 & 1 \\ 
  M71 & Architecture-Engineering & 6 & 10 & 39 & 0 & 4 & 2 & 49 & 0 & 1 \\ 
  M72 & R\&D & 1 & 2 & 52 & 0 & 4 & 3 & 48 & 0 & 1 \\ 
  M73 & Advertising & 1 & 7 & 47 & 0 & 5 & 2 & 48 & 0 & 1 \\ 
  M74\_M75 & Other Science & 1 & 8 & 46 & 0 & 4 & 1 & 50 & 0 & 1 \\ 
  N & Private Administration & 16 & 16 & 23 & 0 & 3 & 2 & 50 & 0 & 1 \\ 
  O84 & Public Administration & 6 & 3 & 45 & 2 & 5 & 2 & 48 & 0 & 1 \\ 
  P85 & Education & 1 & 4 & 50 & 0 & 6 & 8 & 41 & 0 & 1 \\ 
  Q & Health & 1 & 6 & 48 & 0 & 7 & 7 & 41 & 0 & 1 \\ 
  R\_S & Other Service & 1 & 1 & 50 & 5 & 4 & 0 & 51 & 0 & 1 \\ 
  T & Household activities & 0 & 0 & 54 & 2 & 0 & 0 & 55 & 0 & 0 \\ 
   \hline
\end{tabular}
}
\caption{Summary table of critical input ratings by IHS Markit analysts.
Columns below \textit{Input-based rankings} show how often an industry has been rated as critical (score=1), half-critical (score=0.5) or non-critical (score=0) input for other industries, or how often the input was rates as NA.
Columns under \textit{Industry-based rankings} give how often an input has been rated as with 1, 0.5, 0 or NA for any given industry.
Column $n$ indicates the number of analysts who have rated the inputs of any given industry. Industry \textit{T} uses no inputs and is therefore not rated.
} 
\label{tab:ihs_results}

\end{table}

==> NEW VERSION Dynamic COVID Production Network/appendices/validation_apx.tex <==
\section{Details on validation} 
\label{apx:validation}

In this appendix we provide further details about validation (Section~\ref{sec:econimpact} in the main paper). In Appendix~\ref{apx:validation_data} we describe the data sources that we used for validation, and we explain how we made empirical data comparable to simulated data. In Appendix \ref{apx:selectedscenario} we give more details about the selected scenario (Section~\ref{sec:selectedscenarioanalysis} in the main paper). 

\subsection{Validation data}
\label{apx:validation_data}
\begin{itemize}
    \item Index of agriculture (release: 12/08/2020): \url{https://www.ons.gov.uk/generator?format=xls&uri=/economy/grossdomesticproductgdp/timeseries/ecy3/mgdp/previous/v26}
    \item Index of production (release: 12/08/2020): \url{https://www.ons.gov.uk/file?uri=/economy/economicoutputandproductivity/output/datasets/indexofproduction/current/previous/v59/diop.xlsx}
    \item Index of construction (release: 12/08/2020): \url{https://www.ons.gov.uk/file?uri=/businessindustryandtrade/constructionindustry/datasets/outputintheconstructionindustry/current/previous/v67/bulletindataset2.xlsx}
    \item Index of services (release: 12/08/2020): \url{https://www.ons.gov.uk/file?uri=/economy/economicoutputandproductivity/output/datasets/indexofservices/current/previous/v61/ios1.xlsx}
\end{itemize}

All ONS indexes are monthly seasonally-adjusted chained volume measures, based such that the index averaged over all months in 2016 is 100. Although these indexes are used to proxy value added in UK national accounts, they are actually gross output measures, as determining input use is too burdersome for monthly indexes. 

There is not a perfect correspondence between industry aggregates as considered by ONS and in WIOD. For example, the ONS only releases data for the agricultural sector as a whole, without distinguishing between crop and animal production (A01), fishing and aquaculture (A02) and forestry (A03). In this case, when comparing simulated and empirical data we aggregate data from the simulations, using initial output shares as weights. More commonly, there is a finer disaggregation in ONS data than in WIOD. For example, ONS provides separate information on food manufacturing (C10) and on beverage and tobacco manufacturing (C11, C12), while these three sectors are aggregated into just one sector (C10\_C12) in WIOD. In this case, we aggregate empirical data using the weights provided in the indexes of production and services. These weights correspond to output shares in 2016, the base year for all time series. 

Finally, after performing aggregation we rebase all time series so that output in February 2020 takes value 100.



\subsection{Description of the selected scenario}
\label{apx:selectedscenario}

Figure \ref{fig:new_model_april_may_june_facets} shows the recovery path of all industries, both in the model and in the data. Interpretation is the same as in Figure \ref{fig:new_model_april_may_june_all} in the main text. For readability, industries are grouped into six broad categories.

\begin{figure}[H]
    \centering
\includegraphics[width = 1.0\textwidth]{fig/new_model_april_june_facets.pdf}
    \caption{\textbf{Comparison between model predictions and empirical data.} We plot production (gross output) for each of 53 industries, both as predicted by our model and as obtained from the ONS' indexes. Each panel refers to a different group of industries. Different colors refer to production in April and June 2020. Black lines connect the same industry across these three months. All sectoral productions are normalized to their pre-lockdown levels, and each point size is proportional to the steady-state gross output of the corresponding sector.}
        \label{fig:new_model_april_may_june_facets}
\end{figure}

==> NEW VERSION Dynamic COVID Production Network/shockprop_regtab.tex <==


\begin{table}[!htbp] \centering 
\footnotesize
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\\[-1.8ex] & \multicolumn{6}{r}{ \emph{Dependent variable:} $\log( \sum_i x_{i,30})$ } \\ 
\cline{2-7} \\[-1.8ex]
 Shock size: & 40\% & 40\% & 40\% & 80\% & 80\% & 80\% 
 \\ 
Production: & Leontief & IHS2 & Linear & Leontief & IHS2 & Linear 
 \\ 
\hline \\[-1.8ex] 
 $\log (u_{i,0})$ & $-$0.233$^{***}$ & $-$0.114$^{***}$ & 0.008 & $-$0.440$^{***}$ & $-$0.383$^{***}$ & 0.016 \\ 
  & (0.018) & (0.019) & (0.003) & (0.023) & (0.071) & (0.007) \\ 
  & & & & & & \\ 
 $\log (m_{i,0})$ & 0.067 & 0.065 & $-$0.013 & 0.037 & 0.306 & $-$0.025 \\ 
  & (0.038) & (0.041) & (0.007) & (0.049) & (0.150) & (0.014) \\ 
  & & & & & & \\ 
 $\log (x_{i,0})$ & $-$0.006 & $-$0.019$^{***}$ & $-$0.008$^{***}$ & $-$0.011 & $-$0.079$^{***}$ & $-$0.016$^{***}$ \\ 
  & (0.004) & (0.004) & (0.001) & (0.005) & (0.016) & (0.001) \\ 
  & & & & & & \\ 
 Constant & 15.512$^{***}$ & 15.673$^{***}$ & 15.560$^{***}$ & 15.224$^{***}$ & 16.175$^{***}$ & 15.641$^{***}$ \\ 
  & (0.050) & (0.053) & (0.009) & (0.065) & (0.197) & (0.018) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 55 & 55 & 55 & 55 & 55 & 55 \\ 
Adjusted R$^{2}$ & 0.776 & 0.456 & 0.722 & 0.890 & 0.448 & 0.719 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.01; $^{**}$p$<$0.001; $^{***}$p$<$0.0001} \\ 
\end{tabular} 
  \caption{
  \textbf{Regression results for supply shock experiments. \\
  }
  } 
  \label{tab:regsuppshock}
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\\[-1.8ex] & \multicolumn{6}{r}{ \emph{Dependent variable:} $\log( \sum_i x_{i,30})$ } \\ 
\cline{2-7} \\[-1.8ex]
& (1) & (2) & (3) & (4) & (5) & (6) 
 \\ 
\hline \\[-1.8ex] 
 $\log (u_{i,0})$ & 0.040$^{**}$ &  &  &  & 0.012 & 0.036$^{***}$ \\ 
  & (0.010) &  &  &  & (0.010) & (0.008) \\ 
  & & & & & & \\ 
 $\log (m_{i,0})$ &  & 0.021 &  &  & $-$0.024 & $-$0.030 \\ 
  &  & (0.024) &  &  & (0.019) & (0.018) \\ 
  & & & & & & \\ 
 $\log (c_{i,0}+f_{i,0})$ &  &  & $-$0.012$^{***}$ &  & $-$0.011$^{***}$ &  \\ 
  &  &  & (0.002) &  & (0.002) &  \\ 
  & & & & & & \\ 
 $\log (x_{i,0})$ &  &  &  & $-$0.014$^{***}$ &  & $-$0.013$^{***}$ \\ 
  &  &  &  & (0.002) &  & (0.002) \\ 
  & & & & & & \\ 
 Constant & 15.443$^{***}$ & 15.453$^{***}$ & 15.588$^{***}$ & 15.618$^{***}$ & 15.586$^{***}$ & 15.599$^{***}$ \\ 
  & (0.006) & (0.013) & (0.016) & (0.023) & (0.025) & (0.023) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 55 & 55 & 55 & 55 & 55 & 55 \\ 
Adjusted R$^{2}$ & 0.217 & $-$0.004 & 0.522 & 0.452 & 0.522 & 0.580 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.01; $^{**}$p$<$0.001; $^{***}$p$<$0.0001} \\ 
\end{tabular} 
  \caption{
  \textbf{Regression results for demand shock experiments.}
  As representative case we show regression results for the scenario of 60\% shocks to final consumption, because results are similar for alternative shock sizes. Note that economic impacts are identical across alternative production functions. 
  } 
\label{tab:regdemashock} 
\end{table} 








